FRAMER/Miu: Tagged Pointer-based Capability and Fundamental Cost of Memory Safety & Coherence (Position Paper)

Ensuring system correctness, such as memory safety, can eliminate security vulnerabilities that attackers could exploit in the first place. However, high and unpredictable performance degradation remains a primary challenge. Recognizing that it is extremely difficult to achieve complete system correctness for production deployment, researchers make trade-offs between performance, detection coverage, interoperability, precision, and detection timing. This research strikes a balance between comprehensive system protection and the costs required to obtain it, identifies the desirable roles of software and hardware, and presents a tagged pointer-based capability system as a stand-alone software solution and a prototype for future hardware design. This paper presents follow-up plans for the FRAMER/Miu generic framework to achieve these goals.

==> figs/header.tex <==
\usepackage{libertine}
\usepackage{epsfig}
\usepackage{tikz}
\usepackage{amsmath,tabu}
\usepackage{graphicx}
\usepackage{adjustbox}
\usepackage{amssymb,amsmath,enumitem}
\usepackage{fancyvrb}
\usepackage{color,soul}
\usepackage{array,colortbl,xcolor}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepackage{standalone}
\usepackage{url}
\usepackage{subcaption}
\usepackage{fancyvrb}
\usepackage{bussproofs}
\usepackage{setspace, xspace, multirow}
\usepackage{lipsum} % just for the example
\usepackage{xparse}
%   font
%\usepackage{courier}
%\usepackage{PTSansCaption} 

%\usepackage{lmodern}

%\renewcommand{\ttdefault}{pcr}

\usepackage{listings}
\lstset{language=C, 
        mathescape=true, numbers=left,
        xleftmargin=2.2em,xrightmargin=0.3em,
        frame=single,
        framexleftmargin=1.8em, 
        basicstyle=\fontfamily{pcr}\footnotesize, 
        breaklines=true, 
}

% for \lstinline!blah!
%\lstnewenvironment{Ccode}{\lstset{language=C++,basicstyle=\ttfamily\small,numbers=left,numberstyle=\ttfamily\small,columns=flexible,xleftmargin=4em,xrightmargin=4em}}{}
%\lstnewenvironment{MyAssembler}{\lstset{language=[x86masm]Assembler,
%basicstyle=\ttfamily,numbers=left,numberstyle=\small,xleftmargin=4em,xrightmargin=4em}}{}


%%
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
%%


% \texttt font size
\usepackage[scaled=.7]{beramono}

\newbox\verbbox
\usetikzlibrary{patterns}
\usetikzlibrary{decorations.pathmorphing, decorations.pathreplacing,calligraphy}
\usetikzlibrary{positioning,calc, fit}
\usetikzlibrary{shapes,arrows,shadows, shapes.multipart}

\definecolor{myorange}{RGB}{250,192,116}
\definecolor{rred}{HTML}{C0504D}
\definecolor{lgreen}{RGB}{204, 204, 154}
\definecolor{ppurple}{HTML}{9F4C7C}
\definecolor{ggreen}{HTML}{9BBB59}
\definecolor{bblue}{HTML}{4F81BD}
\definecolor{palepurple}{HTML}{F1DAFF}
\definecolor{palemint}{HTML}{CCFFDD}
\definecolor{palegreen}{HTML}{CCEEDD}
\definecolor{palered}{HTML}{FFCCCC}
\definecolor{pastelteal}{HTML}{A6DDCA}
\definecolor{pastelpurple}{HTML}{C7B7D9}
\definecolor{pink}{HTML}{FFF1F2}
\definecolor{skyblue}{HTML}{DBEBF4}
\definecolor{lakeblue}{HTML}{8DBCFF}


% mymodule style
\tikzset{ 
    % default setting (frame)
    helpernode/.style={
        outer sep=0pt, 
        inner sep=0pt,
        node distance=0pt, 
        text width=1cm,
        minimum height=1cm,
        minimum width=1cm,
        trapezium stretches=true,
        rectangle, 
        text=white,
        draw,
    },helpernode/.default=1cm,
    docushape/.style={
        shape=tape,
        %rounded corners=5pt,
        minimum width=5cm,
        inner ysep=3pt,
        draw,
        ultra thick,
        align=center,
        fill=white,
        %font=\fontsize{8}{8}\sffamily\bfseries,
        font=\scriptsize\ttfamily, 
        tape bend top=none,
    },
    arrowstyle/.style={
        single arrow, 
        fill=blue!50, 
        anchor=base, 
        align=center,
        ultra thick,
        text width=2.8cm
    },
    mymodule/.style={
        rounded corners=0.5mm,
        draw=black,
        ultra thick,
        font=\footnotesize\ttfamily, 
        minimum width=2cm,
        minimum height=0.5cm,
      %  inner ysep=1pt
    },
    myshade/.style={
       rounded corners=1mm,
       ultra thick,
       draw=gray,
       %fill opacity=0.1,
       font=\scriptsize\ttfamily, 
       inner ysep=4pt,
       inner xsep=4pt
    },
    mypointer/.style={
       thick,
       draw=black,
       font=\scriptsize\ttfamily, 
    },
     box/.style={
        node distance=0pt,outer sep=0pt,
        draw=black,
        thick,
        fill=white, 
        minimum height=0.5cm,  
        font=\fontsize{8}{8}\ttfamily, 
        anchor=west,
    },
        object/.style={
        rounded corners=1mm,
        draw=black,
        fill=white, 
        %line width=1pt,
        minimum width=1.6cm,
        %minimum height=0.2cm,
        text height=2.0pt,
        text depth=0.5pt,
        font=\fontsize{6}{6}\ttfamily, 
        anchor=west
    },
    frame/.style={
        %font=\fontsize{6}{6}\color{black!50}\ttfamily,
        rounded corners=1mm,
        draw=black,
        %line width=1pt,
        thick,
        font=\scriptsize,%\ttfamily, 
        minimum width=2cm,
        minimum height=0.3cm,
        inner sep=0pt
    },
    rightflat/.style={
        append after command={%
            \pgfextra
            \fill[fill=#1] 
            (\tikzlastnode.south east) 
            [rounded corners] -| 
            (\tikzlastnode.west) |- 
            (\tikzlastnode.north) 
            [sharp corners] -| cycle;
        \draw[rounded corners] 
            (\tikzlastnode.south east) -| 
            (\tikzlastnode.west) |- 
            (\tikzlastnode.north east);
            \endpgfextra},
        minimum width=2cm,
        %minimum height=0.3cm,
        inner sep=1.8pt,
        %text height=2.0pt,
        %text depth=0pt,
        font=\scriptsize,%\ttfamily, 
        thick
    },
    leftflat/.style={
        append after command={%
            \pgfextra
            \fill[fill=#1] 
            (\tikzlastnode.north west) 
            [rounded corners] -| 
            (\tikzlastnode.east) 
            |- (\tikzlastnode.south) 
            [sharp corners] -| cycle;
        \draw[rounded corners] 
            (\tikzlastnode.north west) -| 
            (\tikzlastnode.east) |- 
            (\tikzlastnode.south west);
        \endpgfextra},
        minimum width=2cm,
        %minimum height=0.3cm,
        %inner sep=0pt,
        text height=2.0pt,
        text depth=0.5pt,
        fill=bblue,
        thick
    },
    entry/.style={
        % The shape:
        node distance=0pt,outer sep=0pt,
        %line width=1pt,
        draw=black,
        %rounded corners=1mm,
        text width=#1,
        font={\sffamily\bfseries},
        align=center,
        minimum width=0.1cm,
        minimum height=0.3cm
    },
     bits/.style={
        %rounded corners=1mm,
        %line width=1pt,
        node distance=0pt,
        outer sep=0pt,
        %font=\Large\ttfamily,
        %draw=black,
        text width=#1,
        minimum width=0.5cm,
        align=center,
        %text height=2.4pt,
        %text depth=0pt,
        %font=\fontsize{4}{4}\ttfamily, 
        anchor=west
    }, bits/.default=0.5cm,
}

%%%% BAR GRAPH Setting %%%%%%%%%%%%%%%%%%%%

\pgfplotsset{
  %compat=1.18,
  bargraph/.style={
    xlabel={},
    ylabel={},
    xlabel style={font=\tiny},
    ylabel style={align=center, text width=2.2cm, 
                  font=\sffamily\tiny},
    axis x line*=bottom,
    axis y line*=right,
    enlarge x limits=0.05,
    set layers,
    ybar=0.0pt,
    bar width=0.08cm,
    width=6cm, height=2.3cm, 
    ymin=0, 
    %ymax=6,
    %ytick={0,2,4,6},
    %restrict y to domain*=0:6,
    symbolic x coords={
        %perlbench, bzip2, gcc, mcf, gobmk, 
        %hmmer, sjeng, libquantum, h264ref
        perlbench, bzip2, mcf, hmmer, sjeng, 
        libquantum, h264ref, omnetpp, astar, xalancbmk	 
    },
    xtick={
        %perlbench, bzip2, gcc, mcf, gobmk, 
        %hmmer, sjeng, libquantum, h264ref 
        perlbench, bzip2, mcf, hmmer, sjeng, 
        libquantum, h264ref, omnetpp, astar, xalancbmk	 
    },
    visualization depends on=rawy\as\rawy,
    clip=false,
    legend cell align=left,
    x label style={font=\tiny},
    y label style={font=\tiny},
    xticklabel style={font=\fontsize{4}{4}\bfseries,
        rotate=30,
        anchor=east},
    yticklabel style={font=\fontsize{5}{5}\bfseries},
    ylabel near ticks,
    ymajorgrids, major grid style={draw=gray},
    legend style={
        draw=none,
        fill=none,
        at={(0.85, 0.75)},
        anchor=south, legend columns=-1, 
        font=\fontsize{4.5}{4.5}\ttfamily
    },
    xtick align=inside
  }
}

\def\myheight{3.0cm}
\pgfplotsset{
   %     compat=1.18,
  bargraphcsv/.style={
    xlabel={},
    ylabel={},
    table/col sep=comma,
    axis x line*=bottom,
    axis y line*=right,
    enlarge x limits=0.05,
    set layers,
    ybar=0.0pt,
    bar width=0.08cm,
    width=6cm, height=\myheight, 
    ymin=0, 
    visualization depends on=rawy\as\rawy,
    clip=false,
    legend cell align=left,
    x label style={font=\tiny},
    y label style={font=\tiny},
    xticklabel style={font=\fontsize{4}{4}\bfseries,
        rotate=30,
        anchor=east},
    yticklabel style={font=\fontsize{5}{5}\bfseries},
    ylabel near ticks,
    ylabel style={align=center, text width=\myheight, 
                  font=\sffamily\tiny},
    ymajorgrids, major grid style={draw=gray},
    legend style={
        draw=none,
        fill=none,
        at={(0.8, 0.90)},
        %anchor=south, 
        %legend columns=-1,
        %at={(0.5,0.15)},
        anchor=south,
        legend columns=-1,
        font=\fontsize{4.5}{4.5}\ttfamily
    },
    xtick align=inside
  }
}

\tikzstyle{arrow}=[draw, -latex] 
\def\myshift{0.7cm} 
\def\tblwidth{1.35cm}
\def\tblheight{0.5cm}
\def\bitwidth_dis{0.5cm}

\def\csvpath{/Users/poolmoo/tools/clangllvm/miu.2021.llvm.12.0/evaluation/results/csv_files/normalised/} 

\pgfplotsset{compat=newest}

\pgfkeys{
    /tikz/node distance/.append code={
        \pgfkeyssetvalue{/tikz/node distance value}{#1}
    }
}

\newcommand\widernode[5][myorange]{
    \node[
    #1,
    inner sep=0pt,
    shift=($(#2.south)-(#2.north)$),
    yshift=-\pgfkeysvalueof{/tikz/node distance value},
    fit={(#2) (#3)},
    label=center:{\sffamily\bfseries#4}] (#5) {};
}

% font



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% macro %%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\jin}[1]{\textcolor{red}{Jin: #1}}
\def\miu{Miu}
\def\pname{FRAMER}
\def\miupath{/Users/poolmoo/tools/clangllvm/miu.2021.llvm.12.0/evaluation/results/csv_files/normalised/miu/}
\def\asanpath{/Users/poolmoo/tools/clangllvm/miu.2021.llvm.12.0/evaluation/results/csv_files/normalised/asan/}

% Comment defining
\newcommand{\mycomment}[1]{}

% struct name
\newcommand{\structmdobj}{MDAttachedObjT}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


